BAT X-ray Survey - I: Methodology and X-ray Identification

We applied the Maximum Likelihood method, as an image reconstruction algorithm, to the BAT X-ray Survey (BXS). This method was specifically designed to preserve the full statistical information in the data and to avoid mosaicking of many exposures with different pointing directions, thus reducing systematic errors when co-adding images. We reconstructed, in the 14-170 keV energy band, the image of a 90x90 deg$^2$ sky region, centered on (RA,DEC)=105$^{\circ}$,-25$^{\circ}$, which BAT surveyed with an exposure time of $\sim1$ Ms (in Nov. 2005). The best sensitivity in our image is $\sim0.85$ mCrab or $2.0\times 10^{-11}$ erg cm$^{-2}$. We detect 49 hard X-ray sources above the 4.5 $\sigma$ level; of these, only 12 were previously known as hard X-ray sources ($>$15 keV). Swift/XRT observations allowed us to firmly identify the counterparts for 15 objects, while 2 objects have Einstein IPC counterparts \citep{harris90}; in addition to those, we found a likely counterpart for 13 objects by correlating our sample with the ROSAT All-Sky Survey Bright Source Catalog \citep{voges99}. 7 objects remain unidentified. Analysis of the noise properties of our image shows that $\sim75$% of the area is surveyed to a flux limit of $\sim$1 mCrab. This study shows that the coupling of the Maximum Likelihood method to the most sensitive, all-sky surveying, hard X-ray instrument, BAT, is able to probe for the first time the hard X-ray sky to the mCrab flux level. The successful application of this method to BAT demonstrates that it could also be applied with advantage to similar instruments like INTEGRAL-IBIS.

==> tab.tex <==
\begin{deluxetable}{lccccclccll}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\rotate
\tablecaption{Detected hard X-ray sources \label{tab:src}}
\tablehead{
%%%%%%%% column names
\colhead{SWIFT NAME}               & \colhead{R.A.}       &
\colhead{DEC}            & \colhead{Flux}     &
\colhead{S/N}            & \colhead{Exposure}    & \colhead{ID} & 
\colhead{Offset}         & \colhead{Type}     & 
\colhead{Catalogs\tablenotemark{b}  }     & \colhead{XRT position (ref.)} \\
%%%%%%%%%  units
\colhead{}               & \colhead{\scriptsize (J2000)}  &
\colhead{\scriptsize (J2000)}       & \colhead{\scriptsize(10$^{-11}$ cgs)} &
\colhead{}               & \colhead{\scriptsize{(100 ks) }}         & \colhead{} &
\colhead{\scriptsize(arcmin)}
}
\startdata


J0407.6+0336& 61.9178 & 3.6517 & 4.21  & 5.2  & 330 & 3C 105.0   & 4.7 
  & Sy2 & X  & 04 07 16.2, +03 42 23 \\


J0426.4-5710& 66.6021 & -57.1775 & 2.02  & 4.5 & 803 & 1AXG J042556-5711\tablenotemark{a} & 3.5
 & Sy1 & R  & \nodata \\

J0433.1+0520& 68.2982 & 5.3374 & 7.0  & 10.4  & 316 &  3C 120\tablenotemark{a}  & 1
  & Sy1 & R  & \nodata \\



J0451.6-0349& 72.9205 & -3.8240 & 3.73  & 4.9 & 416 & MCG -01-13-025\tablenotemark{a} & 0.9
  & Sy1.2 & R  & \nodata \\


J0505.8-2351 & 76.4674 & -23.8666 &  2.62  & 7.2 & 816 &   SWIFT J0505.7-2348 & 1.7
  & Sy2 & X  & 05 05 45.4 -23 51 17.0 (1) \\

J0510.8+1631& 77.7224 & 16.5265 & 7.37  & 4.7 & 231  &  CSV 6150\tablenotemark{a}   & 2.5
 & Sy1.5 & R  & \nodata \\

J0514.0-4003 & 78.5146 & -40.0558 & 5.02  & 10.4  &934 & 4U 0513-40 \tablenotemark{a}   & 0.8 
  & LXB & R  & \nodata \\

J0516.0-0007& 79.0096 & -0.1332 & 7.6  & 6.1  & 373 &  QSO B0513-002\tablenotemark{a}  & 2.5
  & QSO-Sy1 & R  & \nodata \\


J0517.1+1633& 79.2839 & 16.5605 & 3.80  & 5.8  &  233  & \nodata &\nodata
 & \nodata & \nodata  & \nodata \\

J0519.5-3240 & 79.8844 & -32.6720 & 4.78  & 8.2  & 909 &  ESO 362- G 018\tablenotemark{a}  & 1.1
  & Sy1.5 & R, X  &  05 19 35.5, -32 39 22 (1)\\

J0519.7-4545 & 79.9460 & -45.7557 & 4.48  & 5.3  & 904 & Pictor A\tablenotemark{a} & 1.5 
  & Sy1 & R  & \nodata \\

J0522.6-3625 & 80.6581  &  -36.4233    & 3.65 & 4.7 &927  &  ESO 362-G021\tablenotemark{a} & 4.6
  & BLLAC &   R, X  & 05 22 57.9, -36 27 29\\



J0529.4-3247 & 82.3541 & -32.7965 & 5.15  & 10.9 & 904  &  V* TV Col\tablenotemark{a} & 1.3
  & CV-DQ* & R  & \nodata \\

J0534.5-5801& 83.6470 & -58.0200 & 1.8 & 5.6 & 800 & V* TW Pic\tablenotemark{a}   & 2.1
  & CV & R, I & \nodata \\

J0539.0-6406 & 84.7717 & -64.1148 & 2.10 & 6.6 &  726  & LMC X-3\tablenotemark{a} & 2.1 
  & HXB & R  & \nodata \\

J0539.5-6943 & 84.8917 & -69.7210 & 4.48 & 8.4 &  681  &LMC X-1\tablenotemark{a} & 1.4 
  & HXB & R, I  & \nodata \\

J0539.9-6919 & 84.9878 & -69.3230 & 6.30 & 8.1  & 681 & PSR B0540-69.3\tablenotemark{a} & 1.4 
  & Pulsar & R, I  & \nodata \\

J0539.9-2842 & 84.9953 & -28.7029 & 5.68  & 4.6  &858  &  PKS 0537-286\tablenotemark{a} &2.5
  & QSO & R, X  & 05 39 54.1, -28 39 54 \\

J0550.8-3215 & 87.7165 & -32.2610 & 3.40  & 6.1 &   883 & PKS 0548-322\tablenotemark{a} & 2.4
  & QSO & R, X  & 05 50 40.4, -32 16 15 \\

J0552.1-0727& 88.0411 & -7.4554 & 32.04  &  33.7 & 477 & NGC 2110   & 0.4
  & Sy2 & X  & 05 52 11.5  -07 27 24  \\


J0558.0-3822 & 89.5237 & -38.3799 & 3.62  & 6.7 & 913 &  LEDA 75476\tablenotemark{a}  & 2.8
  & Sy1 & R  & \nodata \\


J0640.0-2553 & 100.0031 & -25.8931 & 2.54  & 5.3 & 793 &  ESO 490- G 26\tablenotemark{a}  & 2.5
  & Sy1.2 & R, X & 06 40 11.8, 25 53 41 \\



J0727.5-2406 & 111.8951 & -24.1039 & 1.9  & 5.3  & 850 &  \nodata  &\nodata
  & \nodata & R\tablenotemark{e}  & \nodata \\


J0728.6-2604& 112.1626 & -26.0696 &1.87 & 4.7 & 851  & V* V441 Pup\tablenotemark{a} & 3.5
 & HXB & R & \nodata \\


J0731.5+0955& 112.8752 & 9.9214 & 3.30  & 5.9  & 578   &  V* BG CMi  & 1.3
  & CV & E  & \nodata \\


J0732.5-1330& 113.1328 & -13.5037 & 1.85  & 5.9 & 820 & SWIFT J0732.5-1331  & 1.1
  & CV & X & 07 32 37.8, -13 31 07 (3) \\

J0739.6-3144 & 114.9127 & -31.7496 & 2.77  & 6.2  & 846 &  \nodata &\nodata
  & \nodata & \nodata  &  \nodata \\

J0743.0-2543 & 115.7501   & -25.7314 &  1.86 & 5.0 & 869  &  \nodata &\nodata
  & \nodata & R\tablenotemark{e}  &  \nodata \\


J0759.9-3844 & 119.9822 & -38.7422 & 4.90  & 6.0 & 804  &  IGR J07597-3842  &0.5
  & Sy1.2 & R, I, X  & 07 59 41.2, -38 43 57 \\

J0804.2+0507& 121.0552 & 5.1203 & 4.1 & 8.4 & 736  &  UGC 4203\tablenotemark{a}  
& 1.9   & Sy2 & R, X & 08 04 05.4 +05 06 49\\

J0811.5+0937& 122.8750 & 9.6214 & 2.26  & 4.6  & 700 &  \nodata  & \nodata
  & \nodata & R\tablenotemark{d}  & \nodata \\


J0823.3-0456 & 125.8271 & -4.9401 & 3.23  & 8.1 & 846 & SWIFT J0823.4-0457  & 2.0
  & Sy2 & X  & 08 23 01.0, -04 56 02 (3) \\


J0835.3-4510 & 128.8308 & -45.1771 & 17.1  & 22.7 &705 & Vela PSR\tablenotemark{a} & 0.4 
  & PSR & R, I, H  & \nodata \\



J0838.4-3559 & 129.6151 & -35.9976 & 4.01  & 5.5 & 791 &  FRL 1146  &0.7
  & Sy1 & R, I  & \nodata \\

J0839.8-1214& 129.9556 & -12.2467 & 2.43  & 5.8 & 866 & 3C 206\tablenotemark{a}  & 0.4
  & QSO & R  & \nodata \\

 J0844.9-3531 & 131.2411 & -35.5313 & 2.97  & 5.0 & 780  &  \nodata &\nodata
  & \nodata & \nodata  & \nodata \\



J0854.7+1502& 133.6828 & 15.0371 & 5.58  & 5.1 & 646 & \nodata & \nodata
  & \nodata & \nodata  & \nodata \\



J0917.2-6221 &139.112 & -62.359 & 2.07  & 4.5 & 830 & LEDA 90443  & 2.9 
& Sy1 & X & 09 16 08.9, -62 19 29.6 \\



J0918.6+1617& 139.6505 & 16.2987 & 3.3 & 6.7 & 610  &  MRK 0704 & 2.5
  & Sy1.5 & R, X & 09 18 25.9, +16 18 20(3)\\

J0920.3-5512 & 140.0753 & -55.2135 & 9.57  & 15.6  & 612 & 4U 0919-54\tablenotemark{a} & 1.2
  & LXB & R, I, H  & \nodata \\


J0920.8-0805& 140.2134 & -8.0872 & 3.03  & 6.4  &742 & MCG -01-24-012 & 2.2
  & Sy2 & X  & 09 20 46.0, -08 03 21 (2)\\



J0945.9-1421 & 146.4060 & -14.3007 & 5.09  & 5.5 & 621  &  NGC 2992\tablenotemark{a} & 1.5& Sy1.9& R, X  & 09 45 42.1, -14 19 34 \\

J0947.6-3056 & 146.9151 & -30.9388 & 18.01  & 22.8 & 611 &  ESO 434- G 040\tablenotemark{a} &0.6
  & Sy2 & R, I, X  & 09 47 39.8, -30 56 55 \\

J0947.7+0725& 146.9447 & 7.4191 & 5.58  & 4.7   & 581 &  3C 227 & 0.4
  & Sy1 & E,R\tablenotemark{c} & \nodata \\




J0959.5-2251& 149.8805 & -22.8561 & 7.80  & 10.8  & 566 &  NGC 3081\tablenotemark{a}  & 1.8
  & Sy2 & R & \nodata \\


\enddata

\tablenotetext{a}{Source identified thanks to its proximity to a ROSAT Bright
Source with the method described in the text.}

\tablenotetext{b}{Catalogs and Instruments used to identify the source:
R=ROSAT catalog, I= INTEGRAL catalog, H= HEAO-1 catalog, E= Einstein IPC catalog,
X= XRT observations.}



\tablenotetext{c}{3C 227 was detected in a long (11\,ks) ROSAT-PSPC
observations \citep{crawford95}.} 


\tablenotetext{d}{Source J0811.5+0937 has a ROSAT counterpart,
 1WGA J0811.5+0933, reported in the WGA catalog \citep{white94}.
This source coincides with RX J081132.4+093403.}

\tablenotetext{e}{Object has a ROSAT source in the error box, 
however the association has to be proven.}


\tablerefs{ (1) Tueller et al. (2005); (2) Kennea et al. (2005); 
(3) Ajello et al. (2006);
}

\end{deluxetable}

